Detecting Anomalous Activity on Networks with the Graph Fourier Scan Statistic

We consider the problem of deciding, based on a single noisy measurement at each vertex of a given graph, whether the underlying unknown signal is constant over the graph or there exists a cluster of vertices with anomalous activation. This problem is relevant to several applications such as surveillance, disease outbreak detection, biomedical imaging, environmental monitoring, etc. Since the activations in these problems often tend to be localized to small groups of vertices in the graphs, we model such activity by a class of signals that are supported over a (possibly disconnected) cluster with low cut size relative to its size. We analyze the corresponding generalized likelihood ratio (GLR) statistics and relate it to the problem of finding a sparsest cut in the graph. We develop a tractable relaxation of the GLR statistic based on the combinatorial Laplacian of the graph, which we call the graph Fourier scan statistic, and analyze its properties. We show how its performance as a testing procedure depends directly on the spectrum of the graph, and use this result to explicitly derive its asymptotic properties on a few significant graph topologies. Finally, we demonstrate theoretically and with simulations that the graph Fourier scan statistic can outperform naive testing procedures based on global averaging and vertex-wise thresholding. We also demonstrate the usefulness of the GFSS by analyzing groundwater Arsenic concentrations from a U.S. Geological Survey dataset.

==> SSS_ale.tex <==
\section{Graph Fourier Scan Statistic}

In order to derive the Graph Fourier Scan Statistic (GFSS), we will consider specifically the piece-wise constant graph structure, $H^{PC}_1$.
Before we arrive at the GFSS, we recall the Spectral Scan Statistic (SSS).
The SSS was derived originally in \cite{sharpnack2012changepoint}, but since its publication the authors derived the graph Fourier scan statistic.
While the GFSS is shown to be a relaxation of the SSS, we favor the GFSS because it is simple to implement, performs as well as the SSS in practice, and allows for a more exhaustive theoretical analysis.
This has practical implications because p-values and power curves can be derived analytically.

\subsection{Derivation of GFSS}

The hypothesis testing problem with signal in $\Xcal_{PC}(\mu,\rho)$ presents
two challenges: (1) the model contains an unbounded nuisance parameter $\alpha
\in \mathbb{R}$ and (2) the alternative hypothesis is comprised of a finite
disjoint union of composite hypotheses indexed by $\mathcal{C}$. These features
set our problem apart from existing work of structured normal means problems
(see, e.g. \cite{castro:05, arias2008searching,
arias2011detection,addario2010combinatorial}), which does not consider nuisance
parameters and relies on a simplified framework consisting of a simple null
hypothesis and a composite hypothesis consisting of disjoint unions of simple
alternatives. %Having nuisance parameters and composite hypothesis require a more sophisticated analysis.

%We will eliminate the interference caused by the nuisance parameter by considering test procedures that are independent of $\alpha$ (or equivalently $\bar \xb$). 
%The formal justification for this choice is based on the theory of optimal invariant hypothesis testing (see, e.g., \cite{lehmann2005testing}) and of uniformly best constant power tests (see \cite{wald:43}). 
%We will not provide the details and refer the reader to \cite{fouladirad2008optimal,fouladirad2005optimal,fillatre2012,scharf94,baygun.hero:95} and references therein for in depth-treatments of these issues related to the model a hand.

To derive the GFSS we will first consider the simpler problem of testing the null hypothesis that $\xb = \bar \xb$,
i.e. that the signal is constant, versus the alternative composite hypothesis that
\[
    \xb = \alpha \one + \delta \one_C : \alpha, \delta \in
    \RR, \delta \neq 0, 
\]
for one given non-empty $C \subset [p]$. A standard approach to solve this
testing problem is to compute the likelihood ratio (LR) statistic
\begin{equation}
\label{eq:LR}
2 \log \Lambda_C(\yb) = \frac{1}{\sigma^2} \frac{p}{|C| |\bar{C}|} \left( \sum_{v \in C} \tilde{\yb}_v \right)^2,%\frac{1}{2 \sigma^2} (\sum_{v \in C} \tilde y_v^2 - (\tilde y_v - \frac{\one_C^\top \tilde \yb}{|C|})^2 + \sum_{v \in \bar C} \tilde y_v^2 - (\tilde y_v - \frac{\one_{\bar C}^\top \tilde \yb}{|\bar C|})^2) \right)
\end{equation}
where $\tilde \yb = \yb - \bar \yb = (\tilde \yb_v, v \in V)$, 
and to reject the null hypothesis for large values of $ \Lambda_C(\yb)$
(the exact threshold for rejection will depend on the choice of the test significance level). Equation \eqref{eq:LR} was first obtained in
\cite{sharpnack2012changepoint}. In Appendix B, we provide an alternative derivation 
that shows rigorously how we can eliminate the interference caused by the
nuisance parameter by considering test procedures that are independent of
$\alpha$ (or equivalently $\bar \xb$). The formal justification for this choice
is based on the theory of optimal invariant hypothesis testing (see, e.g.,
\cite{lehmann2005testing}) and of uniformly best constant power tests (see
\cite{fouladirad2008optimal,fouladirad2005optimal,fillatre2012,scharf94,baygun.hero:95,wald:43}). 

The same testing procedure (i.e. reject for
large value of the LR \eqref{eq:LR}) can of course be used to test the more
restrictive composite alternative hypothesis that  $\xb \in \Xcal_{PC}(\mu,C)$,
for a fixed non empty $C \subset [p]$ and $\mu>0$. In fact, in Appendix B we
show that the LR statistic yields a less powrful test than the uniformly most powerful test for this
alternative.



%
%For the simpler problem of testing $\xb = \bar \xb$ versus $\xb \in \Xcal_{PC}(\mu,C)$ for some $C \subset V$, the optimal test is based on the likelihood ratio (LR) statistic (see \cite{sharpnack2012changepoint} for a derivation).
%\begin{equation}
%2 \log \Lambda_C(\yb) = \frac{1}{\sigma^2} \frac{p}{|C| |\bar{C}|} \left( \sum_{v \in C} \tilde{\yb}_v \right)^2,%\frac{1}{2 \sigma^2} (\sum_{v \in C} \tilde y_v^2 - (\tilde y_v - \frac{\one_C^\top \tilde \yb}{|C|})^2 + \sum_{v \in \bar C} \tilde y_v^2 - (\tilde y_v - \frac{\one_{\bar C}^\top \tilde \yb}{|\bar C|})^2) \right)
%\end{equation}
%where $\tilde \yb = \yb - \bar \yb = (\tilde \yb_v, v \in V)$. 
%This test rejects $H_0$ for large values of $\Lambda_C(\yb)$. Optimality follows from the fact that the statistical model we consider has the monotone likelihood ratio property.

%\subsection{Spectral Scan Statistic}
When testing against the more complex composite alternative $\xb \in \{
    \Xcal_{PC}(\mu,C), C \in \mathcal{C}(\rho)\}$, for a given $\rho>0$, 
 it is customary to consider instead the generalized likelihood ratio (GLR) statistic, which in our case reduces to
\[
\hat g =  \max_{C \in \mathcal{C}(\rho)} 2 \sigma^2 \log \Lambda_C(\yb).% \textrm{ s.t. } \frac{|\partial C \cap \partial \bar{C}| |V| }{|C||\bar{C}|} \le \rho, C \subset V
\]
With simple algebraic manipulations of the LR statistic \eqref{eq:LR}, we find
that the GLR statistic has a very convenient form which is tied to the spectral
properties of the graph $G$ via its Laplacian. We state it as a result and omit
the simple proof.
\begin{lemma}
\label{lem:GLRTform}
  Let $\Kb = \Ib - \frac{1}{p} \one \one^\top$ and set $\tilde{\yb} = \Kb \yb$. Then
\begin{equation}
\label{eqn:GLRT}
\hat g = \max_{\xb \in \{0, 1\}^p} \frac{\xb^\top \tilde{\yb}\tilde{\yb}^\top \xb}{\xb^\top \Kb \xb} \textrm{ s.t. } \frac{ \xb^\top \Delta \xb}{\xb^\top \Kb \xb} \le \rho,
\end{equation}
where $\Delta$ is the combinatorial Laplacian of the graph $G$.
\end{lemma}

An interesting feature of the GLR statistic is that the program \eqref{eqn:GLRT}
is directly related to the renown sparsest cut problem in combinatorial
optimization. See Section 2 of \cite{sharpnack2012changepoint} for details.

%The proof is provided in Appendix A.
%\js{The following paragraph is from the AISTATS paper verbatim - must change...}
%The savvy reader will notice the connection between \eqref{eqn:GLRT} and the graph sparsest cut program.
%By weak duality, we see that the program \eqref{eqn:GLRT} is bounded by (for some Lagrangian parameter $\nu$) 
%\[
%\min_{C \subseteq V} \frac{\Wb(\partial C)}{|C||\bar C|} - \nu \frac{(\sum_{i \in C} \tilde y_i )^2}{|C||\bar C|}
%\]
%the first term of which is precisely the {\em sparsest cut} objective, and the second term drives the solution $C$ to have positive within cluster empirical correlations.
%The sparsest cut program is known to be NP-hard, with poly-time algorithms known for trees and planar graphs \cite{matula1990sparsest}.
%Because of this fact, approximate algorithms have been proposed over the past two decades, most notably the uniform multicommodity flow approach of \cite{leighton1988approximate,shmoys1997cut} and the semi-definite relaxation of the cut metric \cite{arora2009expander}.
%While it is tempting to apply these same relaxation techniques to \eqref{eqn:GLRT}, the addition of the data driven objective $\tilde \yb \tilde \yb^\top$ renders these approaches invalid. 
%\cite{hagen1992new} observed that the minimum cut sparsity is bounded by the algebraic connectivity ($\lambda_2$), suggesting the Fiedler vector (i.e. the second eigenvector of $\Delta$) to be an appropriate relaxation of the  characteristic vector of the cut.
%Moreover, the well known Cheeger inequality shows that the minimum cut sparsity (in a regular graph) is bounded by the algebraic connectivity (see \cite{chung2004discrete}).
%We will follow the tradition of bounding sparsity with the algebraic connectivity, and provide a surrogate estimator to the scan statistic based on this simple spectral relaxation.

In order to obtain a tractable relaxation of the GLR statistic
\eqref{eqn:GLRT} \cite{sharpnack2012changepoint} introduced the Spectral Scan
Statistic (SSS), defined as
\[
\hat{s} = \sup_{\xb \in \RR^p} (\xb^\top \tilde\yb)^2  \textrm{ s.t. }\xb^\top \Delta \xb \le \rho, \| \xb \| \le 1, \xb^\top \one = 0.
\]
Indeed, \cite{sharpnack2012changepoint} proved that the SSS is an upper bound to
the GLRT statistic:
\begin{proposition}
\label{prop:SSS_def}
The GLR statistic is bounded by the SSS: $\hat g \le \hat s$, almost everywhere.
\end{proposition}

Notice that because the domain $\Xcal = \{ \xb \in \RR^n : \xb^\top \Delta \xb \le \rho, \| \xb \| \le 1, \xb^\top \one = 0 \}$ is symmetric around the origin, this is precisely the square of the solution to
\begin{equation}
\label{eqn:sGP}
\sqrt{\hat{s}} = \sup_{\xb \in \RR^n} \xb^\top \yb  \textrm{ s.t. }\xb^\top \Delta \xb \le \rho, \| \xb \| \le 1, \xb^\top \one = 0,
\end{equation}
where we have used the fact that $\xb^\top \tilde\yb = ( (\Ib - \frac{1}{n}\one \one^\top) \xb )^\top \yb = \xb^\top \yb$ because $\xb^\top \one = 0$ within $\Xcal$. 

\begin{proposition}
\label{prop:GFSS_def}
Recall the definition of the GFSS, $\hat t$ in \eqref{eq:GFSS}.
% \[
% \hat t = \sum_{i = 2}^p \min \left\{1 , \frac{\rho}{\lambda_i} \right\} [(\ub_i^\top \yb)^2 - 1]
% \]
The SSS as a function of $\rho$ can be bounded above and below in the following:
\[
\hat t + \sum_{i = 2}^p \min \left\{1 , \frac{\rho}{\lambda_i} \right\} \le \hat s \le 2 (\hat t + \sum_{i = 2}^p \min \left\{1 , \frac{\rho}{\lambda_i} \right\})
\]
\end{proposition}

The proof is provided in the Appendix.
While it is not obvious that it is important that the GFSS is a relaxation of the GLRT, it is a natural starting point for the development of a suite of changepoint detectors on graphs.
Understanding its performance is an important step in the possibly long process of characterizing the difficulty of distinguishing $H_0$ from $H_1^{PC}$.
It is not clear, even if it is possible to obtain a poly-time algorithm that can distinguish $H_0$ from $H_1^{PC}$ over {\em any} graph under the critical SNR regime.
Let us consider the GFSS and show what it does in our torus example.

\begin{example}{(GFSS for the Torus)}
It has been shown that the Laplacian eigenvalues of the torus graph are $2 (2 - \cos (2 \pi i_1/\ell) - \cos (2 \pi i_2 / \ell))$ for all $i_1,i_2 \in [\ell]$  (see \cite{sharpnack2010identifying} for a derivation).
The eigenvectors correspond to that of the discrete Fourier transform.
So the GFSS for the Torus graph corresponds to the energy of linear shrinkage in the frequency domain.
\end{example}

%In order to quantify the uncertainty inherent in this testing problem, we study the properties of the GFSS.

\subsection{Theoretical Analysis of GFSS}

A thorough theoretical analysis of the GFSS has several uses.
In Corollary \ref{cor:crit_SNR}, we characterize the critical signal-to-noise ratio, enabling us to determine the strength of the GFSS as a detector on theoretical grounds.
%Theorem \ref{thm:main} gives the practicioner ways to quantify the uncertainty inherent in the GFSS, providing a simple way to calculate p-values and power curves without need for computationally expensive simulations from the null hypothesis.
Theorem \ref{thm:main} will be used to form an adaptive version of the GFSS, which will in turn alleviate the need for specifying $\rho$.

The following main result bounds the test statistic under $H_0$ and under the piece-wise constant ($H_1^{PC}$) and the general graph structured ($H_1^S$).
It is based on the concentration of weighted sums of independent $\chi^2$ random variables found in \cite{laurent2000adaptive}.

\begin{theorem}
\label{thm:main}
Under the null hypothesis $H_0$, with probability at least $1 - \alpha$ where $\alpha \in (0,1)$,
\begin{equation}
\label{eq:null_control}
\hat t \le 2 \left( \sqrt{\sum_{i=2}^p \min \{1 , \frac{\rho^2}{\lambda_i^2} \} \log (1 / \alpha) } + \log (1 / \alpha) \right).
\end{equation}
Under the alternative hypotheses, $H^{PC}_1, H^S_1$, with probability at least $1 - \gamma$ where $\gamma \in (0,1)$,
\begin{equation}
\label{eq:alt_control}
\hat t \ge \frac{\mu^2}{2 \sigma^2} - \frac {2\mu} \sigma \sqrt{\log(2 / \gamma)} - 2 \sqrt{\sum_{i=2}^p \min \{1 , \frac{\rho^2}{\lambda_i^2} \} \log(2/\gamma)}.
\end{equation}
\end{theorem}

The proof is provided in the Appendix.
Theorem \ref{thm:main} shows that by setting a threshold to be the right hand side of \eqref{eq:null_control}, we have a level $\alpha$ test.
If we then set the right hand side of \eqref{eq:alt_control} to be this threshold, and solve for $\mu/\sigma$, then we get the lowest SNR such that the test has power $1 - \gamma$ under the alternative.
%Equivalently, we could invert the equations, \eqref{eq:null_control}, \eqref{eq:alt_control}, to obtain p-values and power curves for the GFSS test statistic.
The result below allows us to compare the GFSS to other tests on asymptotic theoretical grounds.

\begin{corollary}
\label{cor:crit_SNR}
The GFSS $\hat t$ can asymptotically distinguish $H_0$ from $H_1^{PC}, H_1^S$ if the SNR is stronger than
\[
\frac{\mu}{\sigma} = \omega \left( \sum_{i = 2}^p \min \{1 , \frac{\rho^2}{\lambda_i^2} \} \right)^{1/4}.
\]
\end{corollary}

Most notably the critical SNR is lower than $p^{1/4}$ which is the critical SNR enjoyed by the energy test statistic.
Comparing this to the analogous results for the SSS in \cite{sharpnack2012changepoint} (Cor.~8), we see that this is a significant improvement.
The most unreasonable assumption that we have made thus far is that the cut sparsity, $\rho$, is known.
This unreasonable advantage is especially apparent when we compare the GFSS to the max and aggregate statistics that do not require the knowledge of $\rho$.
The following section develops a test that adapts to $\rho$.

Before we delve into that, a remark on the computational complexity of the proposed
test is in order. The worst-case runtime of computing all the eigenvalues of a $p\times p$ 
matrix is cubic in $p$. Thus, we have clearly demonstrated a test that is 
computationally feasible for any graph topology i.e. it runs in polynomial (cubic) time 
in the size of the graph $p$, compared to the GLRT whose computation can be exponential
in $p$ in the worst case. However, cubic computational complexity might be prohibitive 
for very large graphs. 
It turns out that the GFSS can be calculated with just the top $j$ eigenvectors and a Laplacian solver.
Specifically, if $j = \max\{ i : \lambda_i < \rho \}$ and let $\Pb_j$ be the projection onto the span of $\{\ub_i\}_{i=2}^p$ then the GFSS can be written as 
\[
\yb^\top \Pb_j \yb + \rho \yb^\top (\Ib - \Pb_j) \Delta^{\dagger} (\Ib - \Pb_j) \yb - \sum_{i = 2}^p \min\big\{ 1 , \frac{\rho}{\lambda_i} \big\}.
\]
The first term requires the computation of the top $j$ eigenspace, while the second term requires a Laplacian solver.
One can observe that the final term is the expected value of the first two terms applied to a vector drawn from the p-dimensional standard normal, indicating that it can be approximated by Monte carlo sampling.
The computation of the first two terms take time $O(k p^2 + m \textrm{polylog}(m))$ by using the fast Laplacian solvers of \cite{koutis2010approaching}.
Furthermore, when the GFSS will be used on multiple measurement vectors (such as multiple measurements in time), then $\Pb_j$ needs to only be computed once. 

\js{I think this can be omitted since what it above is exact.}
In this case, there will be a cost in 
terms of worse statistical performance that will need to be paid for computational efficiency. 
This cost (increase in the risk) can be characterized explicitly in terms of how many 
eigenvalues are used in the computation of the statistic and 
how quickly the eigen-spectrum of the graph Laplacian decays, however this is outside the scope
of this paper. 

\js{Maybe comment on how the filter, once computed, can be used many times.}


==> analysis.tex <==
\section{Theoretical Analysis}

We first derive a simple condition for asymptotic indistinguishability based on testing the null versus a single component in the alternative. 
%While we do not necessarily expect the resulting bound to be sharp, nonetheless it does provides us with a minimal conditions for asymptotic distinguishability.  
A more refined analysis of the lower bound for the general hypothesis \eqref{eq:H0:H1} is beyond the scope of this article. 

\begin{theorem}
\label{thm:lower_bd}
$H_0$ and $H_1$ are asymptotically indistinguishable if $\eta / \sigma = o(1)$.
\end{theorem}

The proof is in the appendix.
We will analyze the performance of the SSS statistic by relying on its representation \eqref{eqn:sGP} as the square of the supremum of a Gaussian process. 
We draw heavily on the theory of the generic chaining, perfected in \cite{talagrand2005generic}, which essentially reduces the problem of computing bounds on the expected supremum of Gaussian processes to geometric properties of its index space.
Recall that, under alternative hypothesis, $\| \betab - \bar \betab\| \geq \eta$ uniformly over $\Theta_1$.

\begin{theorem}
  \label{thm:hypo_bd}
  The following hold with probability at least $1 - \delta$.
  Under the null $H_0$
  \[
  \hat s \le \left( \sqrt{2 \sigma^2 \sum_{i > 1} \min\{1, \rho \lambda_i^{-1}\}} + \sqrt{2 \sigma^2 \log\frac{2}{\delta}} \right)^2,
  \]
  while the alternative $H_1$ %$\yb = \betab + \epsilonb$, for $\frac{\betab - \bar \betab}{\| \betab - \bar \betab \|} \in \Xcal$ and $\| \betab - \bar \betab \| \ge \eta$,
  \[
  \hat s \ge \left( \eta - \sqrt{2 \sigma^2 \log\frac{2}{\delta}} \right)^2.
  \]
\end{theorem}

\begin{proof}
We use generic chaining to control the process $\{ \xb^\top \yb \}_{\xb \in \Xcal}$ appearing in the SSS. 
First, we notice that the index set $\Xcal$ is the intersection of an ellipsoid and the unit ball, which is the intuition behind the following lemma.
%And the index set $\Xcal$ is the intersection of an ellipsoid and the unit ball.  
%The stage is set for our main tool for analyzing the spectral relaxation of the GLRT.
\begin{lemma}
  \label{lem:cheegerBdd}
  %Assume the notation of eqn.~\eqref{eqn:sGP}.
  Let $\Lb$ have spectrum $\{\lambda_i \}_{i=1}^n$. Then under $H_0$,
  \[
  \EE \sup_{\xb \in \Xcal} \xb^\top \yb \le \sqrt{2 \sigma^2 \sum_{i > 1} \min\{1,\rho \lambda_i^{-1}\}}.
  \]
\end{lemma}

The proof is provided in the appendix.
We then can use the well known phenomena, that the supremum of a Gaussian process concentrates around it's expectation (see the appendix).
Hence, by Lemma \ref{lem:gauss_sup_conc} the first statement in Theorem \ref{thm:hypo_bd} holds.
The second statement follows by applying standard concentration results to the univariate Gaussian  $\frac{\betab - \bar \betab}{\| \betab - \bar \betab \|} \yb$ and noticing that $\frac{\betab - \bar \betab}{\| \betab - \bar \betab \|} \in \Xcal$ and $\EE \frac{(\betab - \bar \betab)^\top}{\| \betab - \bar \betab \|} \yb = \| \betab - \bar \betab \| \ge \eta$ under $H_1$.
\end{proof}


As a corollary we will provide sufficient conditions for asymptotic distinguishability that depend on the spectrum of the Laplacian $\Lb$. As we will show in the next section, these conditions can be applied to a number of graph topologies whose spectral properties are known. 

\begin{corollary}
\label{cor:hypo_bd}
  The null and alternative, as described in Thm.~\ref{thm:hypo_bd}, are asymptotically distinguished by $\hat s$ and $g_\nu(\yb)$ if
  \begin{equation}
    \label{eqn:dist_bound1}
  \frac{\eta}{\sigma} = \omega \left(\sqrt{\sum_{i > 1} \min\{1, \rho \lambda_i^{-1}\}} \right)
  \end{equation}
  Other stronger sufficient conditions are
  \begin{equation}
    \label{eqn:dist_bound2}
  \frac{\eta}{\sigma} = \omega \left( \sqrt{ k + \frac{(n - k) \rho}{\lambda_{k + 1}} } \right)
  \end{equation}
  if $k$ is large enough that $\lambda_{k+1} > \rho$.
\end{corollary}

\begin{proof}
To see equation~\eqref{eqn:dist_bound1} we note that, due to Theorem \ref{thm:hypo_bd}, if 
\[
\sqrt{2 \sigma^2 \sum_{i > 1} \min\{1, \rho \lambda_i^{-1}\}} + \sqrt{2 \sigma^2 \log\frac{2}{\delta}} = o \left(\eta - \sqrt{2 \sigma^2 \log\frac{2}{\delta}} \right)
\]
then we attain asymptotic distinguishability by choosing any threshold $\tau$ between, and sufficiently far from, the left and right hand side of the previous display.
To show equation~\eqref{eqn:dist_bound2} we note that by choosing $k$ such that $\lambda_{k+1} > \rho$ we see that 
\[
\sum_{1 < i \le k} \min\{1, \rho \lambda_i^{-1}\} \le k \Rightarrow
\sum_{i > k} \min\{1, \rho \lambda_i^{-1}\} \le (n - k) \frac{\rho}{\lambda_{k+1}}.
\vspace{-.2in}
\]
\vspace{-.1in}
\end{proof}

% \begin{lemma}
%   \label{lem:neg_moment}
% Let $X \in \RR$ be a random variable such that $X \in [0,M]$ almost surely for $M > 0$.  Then
% \[
% \EE \frac{1}{X + 1} \le 1 - \frac{\EE X}{M+1}
% \]
% \end{lemma}

% \begin{proof}{Proof of Lemma \ref{lem:neg_moment}}
% We will argue that $\EE \frac{1}{X + 1}$ subject to $\EE X = \bar X$ and $X \in [0,M]$ a.s.~is maximized by the point masses at $0$ and $M$.
% First, we show by induction that for $n > 0$, for any singular induced measure $\mu_X = \sum_{i=1}^n A_i \delta_{a_i}$ with $\{a_i\}_{i=1}^n \subset [0,M]$, $\{A_i\}_{i = 1}^n \subset \RR$ such that $\sum_{i = 1}^n A_i = 1$ then $\EE \frac{1}{X + 1} \le 1 - \EE X / (M + 1)$.
% We see this by replacing $\mu_X$ with $\tilde \mu_X$ where
% \[
% \tilde \mu_X = A_n ((1 - \frac{a_n}{M}) \delta_0 + \frac{a_n}{M} \delta_M) + \sum_{i=1}^{n-1} A_i \delta_{a_i}
% \]
% Then 
% \[
% \int \frac{1}{x + 1} d\mu_X(x) - \int \frac{1}{x + 1} d \tilde \mu_X(x) = A_n ( (1 - \frac{a_n}{M}) + \frac{a_n}{M(M+1)} - \frac{1}{a_n + 1} ) \ge 0
% \]
% because see that $(1 - \frac{a_n}{M}) + \frac{a_n}{M(M+1)} = 1 - a_n/(M+1) \ge \frac{1}{a_n + 1}$ as the secant line dominates the convex $1 / (a_n + 1)$.
% Critically, the expectation of $X$ doesn't change as we replace $\mu_X$ with $\tilde \mu_X$.
% Hence, if we let our induction parameter be $|\{ a_i \ne 0,M : i>0 \}|$, we have that the maximizing $X$ has point masses at $0$ and $M$.
% Recalling that $\EE X$ remained unchanged, we arrive at the form $\tilde \mu_X = (1 - \frac{\EE X}{M}) \delta_0 + \frac{\EE X}{M} \delta_M$.
% Evaluating our objecting gives us the claim.

% Now, it remains to show this for measures that are non-singular.
% Let $F(x)$ be the CDF of $X$, then the objective is the following Riemann-Stieltjes integral,
% \[
% \EE \frac{1}{X + 1} = \int \frac{d F(x)}{x + 1} = \lim_{n \rightarrow \infty} \int \frac{d F_n(x)}{x + 1}
% \]
% where $F_n$ is a sequence of right continuous piecewise constant functions.
% Specifically, let $P_n$ be a sequence of partitions of size $n$, with mesh tending to $0$, then $F_n$ is constant over the $n$ intervals of the partition such that at the knots $F_n$ evaluates to $F$. 
% But then $F_n$ is the CDF of a random variable, call it $X_n$, with $n$ singularities and takes the form of $\mu_X$ above.
% Also, by keeping the same sequence of partitions, we have that $\lim_{n \rightarrow \infty} \EE X_n = \EE X$.
% Thus, for each $n > 0$, $\int \frac{d F_n(x)}{x + 1} \le 1 - \EE X_n / (M + 1) \rightarrow 1 - \EE X / (M + 1)$.
% Combining these facts, we obtain the lemma.
% \end{proof}

Interestingly, there are no logarithmic terms in \eqref{eqn:dist_bound1} that usually accompany uniform bounds of this type, which is attributed to the generic chaining.
Notice that the left hand side of \eqref{eqn:dist_bound1} is always less than $\sqrt{n-1}$, which we will see characterizes the performance of the naive estimator $\| \tilde \yb \|$.

%\subsection{Energy and Edge Thresholding Detectors}

For comparison, we consider the performance of two naive procedure for detection: the energy detector, which reject $H_0$ if $\| \tilde \yb\|^2$ is too large and the edge thresholding detector, which reject $H_0$ if $\max_{(v,w) \in E} | \yb_v - \yb_w |$ is large.
\begin{theorem}
\label{thm:energy}
 $H_0$ and $H_1$ are asymptotically distinguished by $\| \tilde\yb \|$ if and only if 
\[
\frac{\eta}{\sigma} = \omega(\sqrt{n-1}).
\]  
\end{theorem}
The proof (given in the appendix) is a standard $\chi^2$ analysis.
In \cite{sharpnacksparsistency} the authors examined the problem of exact recovery of cluster boundaries in the graph-structured normal means problem by taking differences between observations corresponding to adjacent nodes.
The following result stems from Theorem 2.1 of \cite{sharpnacksparsistency}, and the fact that $|C||\bar C| / n$ scales like $\min\{|C|,|\bar C|\}$ up to a factor of $2$.
\begin{theorem}
\label{thm:edge_thresh}
$H_0$ and $H_1$ are asymptotically distinguished by $\max_{(v,w) \in E} | \yb_v - \yb_w |$ if
\[
\frac{\eta}{\sigma} = \omega \left(\sqrt{\max_{C \in \Ccal, |C| \le n/2} |C| \log n } \right).
\]
\end{theorem}
If $\Ccal$ contains balanced clusters, i.e. bipartitions $(C,\bar C)$ such that $\frac{|C|}{|\bar C|} \asymp 1$, then this result matches the scaling in Theorem \ref{thm:energy} up to a log factor.


% \begin{corollary}
% $H_0$ and $H_1$ are asymptotically distinguished by $g_\nu(\yb)$ only if 
% \[
% \frac{\eta}{\sigma} = \omega\left( (\sum_{i > 1} \min\{1, \lambda_i^{-1}\})^{1/4} \right)
% \]
% \end{corollary}





==> appdiff.tex <==
4,34c4,34
< \begin{proof}[Proof of Theorem \ref{thm:lower_bd}]
< (a) follows from an application of the Neyman-Pearson lemma to the alternative hypothesis with fixed $C \in \Ccal$.
< (b) Notice that if $H_0$ is indistinguishable from $H_1^{PC}$ then so is it indistinguishable from $H_1^S$.
< For the proof let $\sigma = 1$ as it can be absorbed into the signal size $\mu$.
< Notice that the risk can be bounded by 
< \[
< \begin{aligned}
< R(T) = \sup_{\xb = \bar \xb} \EE [T(\yb) | \xb] + \sup_{\xb \in \Xcal(\mu,\rho)} \EE [1 - T(\yb)|\xb] \\
< \ge \EE [T(\yb) | \xb = 0] + \frac{1}{|\Scal|} \sum_{S \in \Scal} \EE [1 - T(\yb) | \xb = \xb^S] = R^*
< \end{aligned}
< \]
< where $\xb^S = \mu \sqrt{\frac{n}{|S||\bar S|}} \one_S$ and $\Scal \subseteq \Ccal$, to be defined later.
< Then following the same argument of Proposition 3.2 in \cite{addario2010combinatorial} it is easy to show that,
< \[
< R^* \ge 1 - \frac 12 \sqrt{\EE \exp\left\{ \frac{\mu^2}{\sigma^2} Z \right\} - 1}
< \]
< where 
< \[
< Z = \frac{p|S \cap S'|}{\sqrt{|S||\bar S||S'||\bar{S'}|}}
< \] 
< for $S,S'$ drawn independently uniformly from $\Scal$.
< Let $k = \lfloor \sqrt{\lfloor p/(2 c) \rfloor} \rfloor$, and let $S$ be the union of $k$ elements of $\Ccal$ chosen uniformly at random without replacement (and let $S'$ be an IID copy of $S$). 
< Notice that $|S| \le p/2$ and because for all $C \in \Ccal$, $p |\partial C| / (|C||\bar C|) \le \rho / 2$ then $p |\partial S| / (|S||\bar S|) \le \rho$.
< Moreover, $Z$ is stochastically bounded by $|K \cap K'| / \sqrt{|K||K'|}$ where $K, K'$ are chosen independently, uniformly from all $k$-sets of $1,\ldots,m = \lfloor p/|C|\rfloor$.
< Hence, we can apply Proposition 3.4 from \cite{addario2010combinatorial} and determine that $R^* > \gamma$ if 
< \[
< \frac{\mu}{\sigma \sqrt{k}} \le \sqrt{\log \left( 1 + \frac{m \log (1 + 4(1 - \gamma)^2)}{k^2} \right)}
< \]
< Because $k^2 \asymp m$ we have asymptotic indistinguishability if $\mu/\sigma = o(\sqrt{k}) = o(m^{1/4}) = o((p / |C|)^{1/4})$.
< \end{proof}
< \vspace{-.25cm}
---
> % \begin{proof}[Proof of Theorem \ref{thm:lower_bd}]
> % (a) follows from an application of the Neyman-Pearson lemma to the alternative hypothesis with fixed $C \in \Ccal$.
> % (b) Notice that if $H_0$ is indistinguishable from $H_1^{PC}$ then so is it indistinguishable from $H_1^S$.
> % For the proof let $\sigma = 1$ as it can be absorbed into the signal size $\mu$.
> % Notice that the risk can be bounded by 
> % \[
> % \begin{aligned}
> % R(T) = \sup_{\xb = \bar \xb} \EE [T(\yb) | \xb] + \sup_{\xb \in \Xcal(\mu,\rho)} \EE [1 - T(\yb)|\xb] \\
> % \ge \EE [T(\yb) | \xb = 0] + \frac{1}{|\Scal|} \sum_{S \in \Scal} \EE [1 - T(\yb) | \xb = \xb^S] = R^*
> % \end{aligned}
> % \]
> % where $\xb^S = \mu \sqrt{\frac{n}{|S||\bar S|}} \one_S$ and $\Scal \subseteq \Ccal$, to be defined later.
> % Then following the same argument of Proposition 3.2 in \cite{addario2010combinatorial} it is easy to show that,
> % \[
> % R^* \ge 1 - \frac 12 \sqrt{\EE \exp\left\{ \frac{\mu^2}{\sigma^2} Z \right\} - 1}
> % \]
> % where 
> % \[
> % Z = \frac{p|S \cap S'|}{\sqrt{|S||\bar S||S'||\bar{S'}|}}
> % \] 
> % for $S,S'$ drawn independently uniformly from $\Scal$.
> % Let $k = \lfloor \sqrt{\lfloor p/(2 c) \rfloor} \rfloor$, and let $S$ be the union of $k$ elements of $\Ccal$ chosen uniformly at random without replacement (and let $S'$ be an IID copy of $S$). 
> % Notice that $|S| \le p/2$ and because for all $C \in \Ccal$, $p |\partial C| / (|C||\bar C|) \le \rho / 2$ then $p |\partial S| / (|S||\bar S|) \le \rho$.
> % Moreover, $Z$ is stochastically bounded by $|K \cap K'| / \sqrt{|K||K'|}$ where $K, K'$ are chosen independently, uniformly from all $k$-sets of $1,\ldots,m = \lfloor p/|C|\rfloor$.
> % Hence, we can apply Proposition 3.4 from \cite{addario2010combinatorial} and determine that $R^* > \gamma$ if 
> % \[
> % \frac{\mu}{\sigma \sqrt{k}} \le \sqrt{\log \left( 1 + \frac{m \log (1 + 4(1 - \gamma)^2)}{k^2} \right)}
> % \]
> % Because $k^2 \asymp m$ we have asymptotic indistinguishability if $\mu/\sigma = o(\sqrt{k}) = o(m^{1/4}) = o((p / |C|)^{1/4})$.
> % \end{proof}
> % \vspace{-.25cm}
44c44
< %The result now follows by considering all the indicator functions corresponding to the sets in $\mathcal{C}$. 
---
> The result now follows by considering all the indicator functions corresponding to the sets in $\mathcal{C}$. 
53c53
<     this end we recall the arguments from Lemma 7 of AISTATPAPER.
---
>     this end we recall the arguments from Lemma 7 of \cite{sharpnack2012changepoint}.
108,109c108,109
<     \sup_{\{ \xb \in \mathbb{R}^p \colon \xb^\top \Ub \Ab' \Ub^\top \xb \le 1 \}}  \yb^\top \xb \le \sqrt{\hat s}
<     \le \sup_{\{ \xb \in \mathbb{R}^p \colon \xb^\top \Ub \Ab' \Ub^\top \xb \le 2\}}  \yb^\top \xb,
---
>     \sup_{\{ \zb \in \mathbb{R}^p \colon \zb^\top \Ub \Ab' \Ub^\top \zb \le 1 \}}  \yb^\top \zb \le \sqrt{\hat s}
>     \le \sup_{\{ \zb \in \mathbb{R}^p \colon \zb^\top \Ub \Ab' \Ub^\top \zb \le 2\}}  \yb^\top \zb,
111,113c111,113
< since every $\zb \in \mathbb{R}^{p-1}$ can be written as $\Ub^\top \xb$ for some
< $\xb \in \mathbb{R}^p.$\footnote{In fact, $\zb = \Ub^\top \xb_1 =  \Ub^\top \xb_2
< $ if and only if the difference $\xb_1 - \xb_2$ belongs to the linear  subspace of
---
> since every $\zb \in \mathbb{R}^{p-1}$ can be written as $\Ub^\top \zb$ for some
> $\zb \in \mathbb{R}^p.$\footnote{In fact, $\zb = \Ub^\top \zb_1 =  \Ub^\top \zb_2
> $ if and only if the difference $\zb_1 - \zb_2$ belongs to the linear  subspace of
116,118c116,134
< Evaluating these programs (one can use the Fenchel dual of indicators over
< ellipsoids) produces the claim.
< \textcolor{red}{{\bf ATTN: give details of the derivation}}
---
> All that remains is to show that 
> \[
> \hat t = \sup_{\{ \zb \in \mathbb{R}^p \colon \zb^\top \Ub \Ab' \Ub^\top \zb \le 1 \}} \yb^\top \zb.
> \]
> This can be seen by strong duality for convex programs,
> \[\begin{aligned}
> \sup_{\{ \zb \in \mathbb{R}^p \colon \zb^\top \Ub \Ab' \Ub^\top \zb \le 1 \}} \yb^\top \zb = \sup_{\{ \zb \in \mathbb{R}^p \colon \zb^\top \Ab' \zb \le 1 \}} (\Ub^\top \yb)^\top \zb \\
> =  \sup_{\{ \zb \in \mathbb{R}^{p-1} \}} \inf_{\eta \ge 0} (\Ub^\top \yb)^\top \zb - \eta (\zb^\top \Ab' \zb - 1)\\
> = \inf_{\eta \ge 0} \sup_{\{ \zb \in \mathbb{R}^{p-1} \}} (\Ub^\top \yb)^\top \zb - \eta (\zb^\top \Ab' \zb - 1).
> \end{aligned}
> \]
> The RHS is maximized at $\zb = (2 \eta \Ab')^{-1} (\Ub^\top \yb)$, and plugging this in it becomes
> \[\inf_{\eta \ge 0} (\Ub \yb)^\top (4 \eta \Ab')^{-1} (\Ub^\top \yb) + \eta
> \]
> which is minimized at 
> \[
> \eta = \sqrt{ (\Ub \yb)^\top (4 \Ab')^{-1} (\Ub \yb) }.
> \]
> Plugging this in completes our proof.
135a152
> Recall the notation of the proof of Prop.~\ref{prop:GFSS_def}.
139c156,161
< \hat t = \yb^\top \Ab \yb - \tr \Ab = \xb^\top \Ab \xb + 2 \xb^\top \Ab \epsilonb + \epsilonb^\top \Ab \epsilonb- \tr \Ab
---
> \begin{aligned}
> &\hat t = \yb^\top \Ub (\Ab')^{-1} \Ub^\top \yb - \tr (\Ab')^{-1} \\
> &= \xb^\top \Ub (\Ab')^{-1} \Ub^\top \xb + 2 \xb^\top \Ub (\Ab')^{-1} \Ub^\top \epsilonb \\
> &\quad + \epsilonb^\top \Ub (\Ab')^{-1} \Ub^\top \epsilonb- \tr (\Ab')^{-1}\\
> &\overset{d}{=} \xb^\top \Ub (\Ab')^{-1} \Ub^\top \xb + 2 \xb^\top \Ub (\Ab')^{-1} \epsilonb + \epsilonb^\top (\Ab')^{-1} \epsilonb- \tr (\Ab')^{-1}\\
> \end{aligned}
141c163
< where $\Ab = \Ub \diag(\{\min\{1,\rho/\lambda_i\}\}_{i=2}^p) \Ub^\top$.
---
> where $\overset{d}{=}$ denotes equality in distribution (which follows from rotational invariance of the isonormal Gaussian).
144,151c166
< \xb^\top \Ab \epsilonb \ge - \sqrt{2 \xb^\top \Ab^2 \xb \log (1 / \alpha)}
< \]
< Because $\Ab$ is positive definite with eigenvalues bounded by $1$, we have that $\xb^\top \Ab^2 \xb \le \xb^\top \Ab \xb$.
< We will now show that $\xb^\top \Ab \xb \ge \mu^2 / 2$ under $H^{PC}_1, H^S_1, H^E_1$.
< Recall that by Fenchel conjugacy, \textcolor{red}{Does it really follow from Fenchel
< conjugacy or just from the definition of dual norm?}
< \[
< \xb^\top \Ab \xb = \sup_{\zb^\top \Ab^\dagger \zb \le 1} (\zb^\top \xb)^2,
---
> \xb^\top \Ub (\Ab')^{-1} \epsilonb \ge - \sqrt{2 \xb^\top \Ub (\Ab')^{-2} \Ub^\top \xb \log (1 / \alpha)}
153,155c168,174
< where $\Ab^\dagger = \Ub \diag(\{\max\{1,\lambda_i / \rho\}\}_{i=2}^p)
< \Ub^\top$.
< 
---
> Because $\Ub (\Ab')^{-1}\Ub^\top$ is positive definite with eigenvalues bounded by $1$, we have that $\xb^\top \Ub (\Ab')^{-2} \Ub^\top \xb \le \xb^\top \Ub (\Ab')^{-1} \Ub^\top \xb$.
> We will now show that $\xb^\top \Ub (\Ab')^{-1} \Ub^\top \xb \ge \mu^2 / 2$ under $H^{PC}_1, H^S_1, H^E_1$.
> Recall that by the dual norm (as derived in the proof of Prop.~\ref{prop:GFSS_def}), 
> %\textcolor{red}{Does it really follow from Fenchel conjugacy or just from the definition of dual norm?}
> \begin{equation}\label{eq:dual_ellipse}
> \xb^\top \Ub \Ab' \Ub^\top \xb = \sup_{\zb^\top \Ub (\Ab')^\dagger \Ub^\top \zb \le 1} (\zb^\top \xb)^2.
> \end{equation}
159c178
< \frac{(\xb - \bar\xb)^\top}{\| \xb - \bar \xb\|} \Lambda \frac{(\xb - \bar\xb)}{\|\xb - \bar \xb\|} \le \rho
---
> \frac{(\xb - \bar\xb)^\top}{\| \xb - \bar \xb\|} \Ub \Lambda \Ub^\top \frac{(\xb - \bar\xb)}{\|\xb - \bar \xb\|} \le \rho
161,162c180,182
< while $\| (\xb - \bar \xb) / \| \xb - \bar \xb \| \| = 1$. \textcolor{red}{Ale:
<     I am a bit confused.  About the dimensions here: $\xb$ is in $\mathbb{R}^p$ but $\Lambda$ has dimension $p-1$.}
---
> while $\| (\xb - \bar \xb) / \| \xb - \bar \xb \| \| = 1$. 
> %\textcolor{red}{Ale:    I am a bit confused.  About the dimensions here: $\xb$ is in $\mathbb{R}^p$ but $\Lambda$ has dimension $p-1$.}
> %\js{Using $\Ub$ as you had it in the previous proof should resolve that.}
165c185
< \frac{(\xb - \bar\xb)^\top}{\| \xb - \bar \xb\|} \Ab^\dagger \frac{(\xb -
---
> \frac{(\xb - \bar\xb)^\top}{\| \xb - \bar \xb\|} \Ub \Ab' \Ub^\top \frac{(\xb -
168c188
<   So,
---
> So,
171,172c191,193
< \frac{(\xb - \bar\xb)^\top}{\sqrt 2 \| \xb - \bar \xb \|} \Ab \frac{(\xb - \bar\xb)}{\sqrt 2 \| \xb - \bar \xb \|} \le 1 \\
< \Rightarrow \xb^\top \Ab \xb \ge \left(\frac{(\xb - \bar\xb)^\top}{\sqrt 2 \| \xb - \bar \xb \|} \xb \right)^2 = \| \xb - \bar \xb\|^2 / 2 \ge \mu^2 / 2
---
> &\frac{(\xb - \bar\xb)^\top}{\sqrt 2 \| \xb - \bar \xb \|} \Ub \Ab' \Ub^\top \frac{(\xb - \bar\xb)}{\sqrt 2 \| \xb - \bar \xb \|} \le 1 \\
> &\Rightarrow \xb^\top \Ub (\Ab')^{-1} \Ub^\top \xb \ge \left(\frac{(\xb - \bar\xb)^\top}{\sqrt 2 \| \xb - \bar \xb \|} \xb \right)^2 \\
> &= \| \xb - \bar \xb\|^2 / 2 \ge \mu^2 / 2
174a196
> by substituting $z = (\xb - \bar \xb) / \sqrt 2 \|\xb - \bar \xb\|$ in \eqref{eq:dual_ellipse}.
178c200,202
< So, $\Kb_C \xb = \frac{\one_C^\top \xb}{|C|} \one_C + \frac{\one_{\bar C}^\top \xb}{|\bar C|} \one_{\bar C}- \bar \xb$.
---
> So, \[
> \Kb_C \xb = \frac{\one_C^\top \xb}{|C|} \one_C + \frac{\one_{\bar C}^\top \xb}{|\bar C|} \one_{\bar C}- \bar \xb.
> \]
180c204,207
< Let $\bar \xb_C = \frac{\one_C^\top \xb}{|C|} \one_C$ and $\bar \xb_{\bar C} = \frac{\one_{\bar C}^\top \xb}{\bar C|} \one_{\bar C}$.
---
> Let 
> \[
> \bar \xb_C = \frac{\one_C^\top \xb}{|C|} \one_C \quad {\rm and }\quad \bar \xb_{\bar C} = \frac{\one_{\bar C}^\top \xb}{|\bar C|} \one_{\bar C}.
> \]
184c211
< = \frac {|\bar C|} n (\bar \xb_C - \bar \xb_{\bar C})
---
> = \frac {|\bar C|} n (\bar \xb_C - \bar \xb_{\bar C}).
192c219
< = \frac{|C||\bar C|}{n} (\bar \xb_{\bar C} - \bar \xb_{C})^2 \ge \mu^2  
---
> = \frac{|C||\bar C|}{n} (\bar \xb_{\bar C} - \bar \xb_{C})^2 \ge \mu^2.
197c224
< The error bound, \eqref{eq:alt_control} follows from these facts and the Lemma \ref{lem:chi_squared} applied to $\epsilonb^\top \Ab \epsilonb - \tr \Ab$.\end{proof}
---
> The error bound, \eqref{eq:alt_control} follows from these facts and the Lemma \ref{lem:chi_squared} applied to $\epsilonb^\top (\Ab')^{-1} \epsilonb - \tr (\Ab')^{-1}$.\end{proof}
276c303
< We should argue the choice of $\rho \propto p^{2k - \ell - 1}$, by showing that it is the results of cuts at level $k$.
---
> We should argue the choice of $\rho \asymp p^{2k - \ell - 1}$, by showing that it is the results of cuts at level $k$.
314d340
< 


==> lemma6_details.tex <==
\begin{proof}[Proof of Lemma \ref{lem:GLRTform}]

    \textcolor{red}{{\bf This is an alternative proof. Let's talk about this}}

    Recall from equation \eqref{eq:X.CP} that any $\xb \in
    \mathcal{X}_{CP}(\mu,C)$
    can be represented as
    \[
	\xb = \alpha \one + \delta \one_C
	\]
	where $\alpha \in \mathbb{R}$ is a nuisance parameter and $\delta \geq
	\mu \sqrt{ \frac{p}{|C||\bar C|} }$. \textcolor{red}{{\bf ATTN: the
	restriction on $\delta$ is not inconsequential and will change the LR! From now on I
    will ignore restriction on $\delta$. The difference actually matters. See
comments below.}}
To eliminate the dependence on the nuisance parameter $\alpha$ and simplify the
problem we will resort to invariant testing theory (REFERENCE TO LEHMAN
CASELLA). In fact, the testing problem remains invariant under the action of
the group of translations,  i.e.  additions of constant vectors, of
the mean of $\yb$. To take
advantage of such invariance we proceed as follows.  Let $Wb$ be a $(p-1) \times p$ whose rows form an orthonormal basis for
$\mathcal{R}^\bot(\one)$, the linear subspace of $\mathbb{R}^P$ orthogonal to the subspace of vectors in $\mathbb{R}^p$ with constant
entries. Then, a maximal invariant with respect with respect to such a group is the $(p-1)$-dimensional random vector
\[
\zb := \Wb \yb = \Wb \one_C \delta + \Wb \epsilonb.
    \]
 Since $\Wb\Wb^\top =
    \Ib_{p-1}$,  $\zb$ as a $N_{p-1}(\Wb \one_C \delta, \sigma^2 \Ib_{p-1})$
distribution, which no longer depends on the nuisance parameter $\alpha$.
Our hypothesis testing problem is then equivalent to the problem of testing $H_0
\colon \mathbb{E}[\zb] = 0$ versus the alternative $H_C \colon \mathbb{E}[\zb] =
\Wb \one_C$. It is also worth pointing out that, as our calculations below show,
the choice of the orthonormal basis of $\mathcal{R}^\bot(\one)$ comprising the
rows of the matrix $\Wb$ does not matter in the construction of the
optimal test.

 To test whether $H_0$
of $H_C$ holds we just compute the LR based on the distribution of $\zb$.
\textcolor{red}{{\bf
    ATTN: if we are testing $H_0 \colon \delta = 0$ versus $H_C \colon \delta \neq
    0$ then the LR we have below is correct. But if the testing problem is  $H_0
    \colon \delta = 0$ versus $H_C \colon \delta \geq
	\mu \sqrt{ \frac{p}{|C||\bar C|} }$, which is what we actually seem to claim,
    then the LR is wrong and we should end up instead with a $\chi^2$.}} 

The LR ($H_1/H_0)$ is
\[
    \frac{\sup_{\delta \in \mathbb{R}} \exp \left\{ -\frac{1}{2 \sigma^2} \left\|\zb - \Wb \one_C \delta
\right\|^2  \right\} }{ \exp\left\{
    - \frac{1}{2 \sigma^2} \| \zb \|^2
\right\}}.
    \]
    Simple calculations yield that MLE of $\delta$ under the alternative is $\frac{\zb^\top \Wb\one_C}{\| \Wb
    \one_C \|^2}$. As a result, the LR becomes
    \[
	\exp\left\{ -\frac{1}{2 \sigma^2} \left[ \left\| \zb - \Wb\one_C \frac{\zb^\top
	\Wb\one_C}{\| \Wb\one_C \|^2} \right\|^2  - \| \zb \|^2 \right]
    \right\},
    \]
which is equal to 
\begin{equation}\label{eq:LR}
    \exp\left\{ \frac{1}{2 \sigma^2} \frac{( \zb^\top\Wb\one_C)^2 }{\| \Wb\one_C\|^2 }
\right\}.
    \end{equation}
We now rewrite the previous display in a simpler form. We have 
\begin{eqnarray*}
\zb^\top \Wb \one_C^\top &  = &  \yb^\top \Wb^\top \Wb \one_C\\
& = & \one_C^\top \Pb_{\one^\bot} \yb\\
& = & \one_C^\top \tilde \yb\\
& = & \sum_{i \in C} \tilde \yb_i,
\end{eqnarray*}
where $\Pb_{\one^\bot} = \Ib_p - \frac{\one \one^\top}{p}$ is the orthogonal projector into the subspace of
$\mathbb{R}^p$ orthogonal to the linear subspace spanned by the constant vectors.  
Next, since $\Pb_{\one^\bot}$ is idempotent, we have 
\begin{eqnarray*}
\| \Wb \one_C \|^2 & = & \one_C^\top \Pb_{\one^\bot} \one_C\\
& = & \|  \Pb_{\one^\bot} \one_C\|^2\\
& = & \sum_{i \in C} \left( 1 - \frac{|C|}{p} \right)^2 + \sum_{i \in \bar C}
\left( - \frac{|\bar C|}{p} \right)^2\\
& = & |C| + \frac{|C|^2}{p^2}|C| - 2\frac{|C|^2}{p} + |\bar C|\frac{ |C|^2}{p^2}\\
& = & \frac{|C|^2}{p^2}(|C| + |\bar C|) + |C| -2 \frac{ |C|^2}{p}\\
& = & |C| - \frac{|C|^2}{p}\\
& = & \frac{|C|(p - |C|)}{p}\\
& = & \frac{|C||\bar C|}{p},\\
    \end{eqnarray*}
where in the above
equalities we repeatedly used the fact that $|C| + |\bar C| = p$. Plugging into
\eqref{eq:LR},
we arrive at the following expression for the log-likelihood ratio
$\Lambda_C(\yb)$: 
\[
2 \sigma^2 \log \Lambda_C(\yb) =\frac{p}{|C| |\bar{C}|} \Big( \sum_{i \in C}
\tilde{\yb}_i \Big)^2. 
    \]
    \textcolor{red}{First we notice that $H_0$ and $H^C_1$ are invariant to a group action that will allow us to simplify the LR statistic.
Let the group action on $\xb \in \RR^n$ be 
\[
G = \{\xb \mapsto \xb + \zb : \frac{1}{|C|} \sum_{v \in C} \zb_v = \frac{1}{|\bar C|} \sum_{v \in \bar C} \zb_v = 0, \zb \in \RR^n\}
\]
We now are able to obtain the maximal invariant statistics to $G$, $\yb_0 = \frac{1}{|C|} \sum_{i \in C} \yb_i \sim N(\beta_0,\sigma_0^2)$ and $\yb_1 = \frac{1}{|\bar C|} \sum_{i \in \bar C}\yb_i \sim N(\beta_1, \sigma_1^2)$ for $\sigma_0 = \sigma / \sqrt{|C|}$ and $\sigma_1 = \sigma / \sqrt{|\bar{C}|}$. 
By the theory of most powerful invariant tests we can reduce the LR statistic for $\yb$ to it's maximal invariants $\yb_0,\yb_1$.
Then, we obtain
\[
 2 \log \Lambda_C(\yb) = \frac{1}{\sigma_0^2} (\yb_0 - \hat{\beta})^2 + \frac{1}{\sigma_1^2} (\yb_1 - \hat{\beta})^2 
\]
where $\hat{\beta} = \frac{\sigma_1^2}{\sigma_0^2 + \sigma_1^2} \yb_0 + \frac{\sigma_0^2}{\sigma_0^2 + \sigma_1^2} \yb_1$ is the MLE under $H_0$. (The likelihood under the alternative balances with the normalizing constant of the null likelihood.) Thus,
\[
 2 \sigma^2 \log \Lambda_C(\yb) = \frac{\sigma^2}{\sigma_0^2} \left( \frac{\sigma_0^2 (\yb_0 - \yb_1) }{\sigma_0^2 + \sigma_1^2} \right)^2 + \frac{\sigma^2}{\sigma_1^2} \left( \frac{\sigma_1^2 (\yb_0 - \yb_1) }{\sigma_0^2 + \sigma_1^2} \right)^2
\]
\[
= \sigma^2 \frac{(\yb_0 - \yb_1)^2}{\sigma_0^2 + \sigma_1^2} = \frac{|C| |\bar{C}|}{|V|} (\yb_0 - \yb_1)^2
\]
\[
= \frac{|V|}{|C| |\bar{C}|} \left( \frac{|\bar{C}|}{|V|}\sum_{v \in C} \yb_v - \frac{|C|}{|V|} \sum_{v \in \bar{C}} \yb_v \right)^2
\]
\[
= \frac{|V|}{|C| |\bar{C}|} \Big( \sum_{v \in C} \yb_v - \frac{|C|}{|V|} \sum_{v \in V} \yb_v \Big)^2 = \frac{|V|}{|C| |\bar{C}|} \Big( \sum_{v \in C} \tilde{\yb}_v \Big)^2.
\]}
Now we let $\xb = {\bf 1}_C$, making the statistic above
\[
2 \sigma^2 \log \Lambda_C(\yb) = \frac{\xb^\top \tilde \yb \tilde \yb \xb}{\xb^\top \Kb \xb} \textrm{ and } \frac{\Wb(\partial C) |V| }{|C||\bar{C}|} = \frac{\xb^\top \Delta \xb}{\xb^\top \Kb \xb}.
\]
The result now follows by considering all the indicator functions corresponding to the sets in $\mathcal{C}$. 
\end{proof}
\vspace{-.25cm}

